Peerify: Benchmarking Peer-Review Claim Verification

Peer review plays a central role in scholarly publishing, yet verifying whether reviewer claims are supported by manuscript evidence remains a largely manual and time-consuming process. We present Peerify, a pipeline for manuscript-grounded verification of peer-review claims. Given a manuscript and a review comment, the Peerify pipeline decomposes reviews into atomic claims, retrieves relevant manuscript evidence, and determines whether each claim is supported by the paper. To support the development and evaluation of the pipeline, we construct a benchmark of 800 claims derived from authentic peer-review interactions collected from NeurIPS 2024 and ICLR 2024, including a 300-claim hand-labeled subset used to audit the automated supervision. We evaluate state-of-the-art language models and retrieval strategies within the Peerify pipeline, together with entailment baselines. Our results demonstrate the importance of retrieval-centered verification and claim decomposition, while highlighting the challenges posed by ambiguous and interpretive reviewer claims. Automated labels agree with human consensus on 90.3% of audited claims ($\kappa = 0.87$), while off-the-shelf entailment models stay below 0.24 macro-F1.

==> Tables/PredDist.tex <==
\begin{table}[t]
\centering
\caption{Predicted label distribution (\%) on \textsc{RebuttalSourced} (B2, full-context) for all five models vs.\ the ground-truth (GT) label distribution. Models whose predicted distribution deviates substantially from GT inflate accuracy through distribution matching rather than genuine reasoning.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Supported} & \textbf{Part.\ Supp.} & \textbf{Contradicted} & \textbf{Not Det.} \\
\midrule
GT (B2) & 27.1 & 38.8 & 23.6 & 10.5 \\
\midrule
\texttt{o4-mini}      & 30.5 & \phantom{0}4.9 & 42.4 & 22.2 \\
\texttt{GPT-5-mini}   & 31.1 & 16.2           & 45.8 & \phantom{0}6.9 \\
\texttt{Claude-Haiku} & 17.2 & 11.6           & \textbf{60.0} & 11.1 \\
\texttt{Qwen3-8B}     & 25.6 & \textbf{60.5}  & 11.1 & \phantom{0}2.8 \\
\texttt{Qwen2.5-7B}   & \textbf{26.9} & \textbf{37.2} & \textbf{21.0} & 14.5 \\
\bottomrule
\end{tabular}%
}
{\footnotesize Bold marks values closest to GT proportion (Supported, PS) or largest over-prediction (Contradicted). \texttt{Qwen2.5-7B} computed on 718 claims (9 papers exceeded its context window).}
\label{tab:pred-dist}
\end{table}


==> Tables/RQ1.tex <==
\begin{table*}[ht]
  \centering
  \caption{RQ1. Performance of Claim-Extraction Models across Datasets and Approaches}
  \label{tab:rq1_results}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{lllcrrrr}
    \toprule
    \textbf{Dataset} & \textbf{Model} & \textbf{Approach} & \textbf{\#Claims} &
    \textbf{Atomicity} & \textbf{Fluency} & \textbf{Decontext.} &
    \textbf{Precision -- Recall} \\
    \midrule

    % ========================= GOLDEN =========================
    \multirow{8}{*}{Golden}

      & FENICE & Ref-Free & 873
      & 0.298 & 0.747 & 0.369 & --- \\

      & Gemma & Ref-Free & 3383
      & 0.366 & 0.763 & 0.296 & --- \\

      & ClaimGuard/T5-multitask-veracity-small & Ref-Free & ---
      & --- & --- & --- & --- \\

    \cmidrule(lr){2-8}

      & FENICE & Ref-Based (Cosine) & 873
      & --- & --- & --- & 0.756 -- 0.660 \\

      & FENICE & Ref-Based (VLLM) & 873
      & --- & --- & --- & 0.843 -- 0.436 \\

      & Gemma & Ref-Based (Cosine) & 3383
      & --- & --- & --- & 0.764 -- 0.619 \\

      & Gemma & Ref-Based (VLLM) & 3383
      & --- & --- & --- & 0.852 -- 0.753 \\

      & ClaimGuard/T5-multitask-veracity-small & Ref-Based & ---
      & --- & --- & --- & --- \\

    \midrule

    % ========================= FEVER =========================
    \multirow{4}{*}{FEVER}

      & FENICE & Ref-Free & ---
      & --- & --- & --- & --- \\

      & Gemma & Ref-Free & ---
      & --- & --- & --- & --- \\

      & ClaimGuard/T5-multitask-veracity-small & Ref-Free & ---
      & --- & --- & --- & --- \\

    \cmidrule(lr){2-8}

      & FENICE & Ref-Based & ---
      & --- & --- & --- & --- \\

      & Gemma & Ref-Based & ---
      & --- & --- & --- & --- \\

      & ClaimGuard/T5-multitask-veracity-small & Ref-Based & ---
      & --- & --- & --- & --- \\

    \bottomrule
  \end{tabular}
  }
\end{table*}


==> Tables/hv_150_vs_300.tex <==
\begin{table}[t]
\centering
\caption{Verification accuracy on the original 150-instance \textsc{Human-Verified} subset versus the expanded 300-instance subset used throughout the camera-ready. FC is full-context; RAG is the best of the four retrievers. Doubling the human-annotated coverage leaves the model ordering and the difficulty level of the split intact.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{2}{c}{\textbf{Full-Context}} & \multicolumn{2}{c}{\textbf{RAG (best retriever)}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\textbf{Model} & $n{=}150$ & $n{=}300$ & $n{=}150$ & $n{=}300$ \\
\midrule
\texttt{o4-mini}      & 0.276 & 0.267 & 0.260 & 0.257 \\
\texttt{GPT-5-mini}   & 0.336 & 0.317 & 0.313 & 0.297 \\
\texttt{Claude-Haiku} & 0.269 & 0.300 & 0.267 & 0.300 \\
\texttt{Qwen3-8B}     & 0.316 & \textbf{0.377} & 0.300 & 0.297 \\
\texttt{Qwen2.5-7B}   & 0.249 & 0.256 & \textbf{0.367} & \textbf{0.340} \\
\bottomrule
\end{tabular}%
}
\label{tab:hv-150-vs-300}
\end{table}


==> Tables/token_usage.tex <==
\begin{table}[h]
\centering
\caption{Average token usage per claim for RAG-based verification across different retrievers and benchmarks.}
\label{tab:rag_tokens}
\begin{tabular}{lcccc}
\toprule
\textbf{Benchmark} & \textbf{BM25} & \textbf{FAISS} & \textbf{Bi-enc + Cross} & \textbf{BM25 + Cross} \\
\midrule
Golden Supported & 2,235.85 & 2,231.82 & 2,384.76 & 2,291.40 \\
Author--Reviewer & 2,156.78 & 2,128.87 & 2,371.78 & 2,236.87 \\
Paper + O4-mini & 2,156.78 & 2,128.87 & 2,371.78 & 2,236.87 \\
Agreement & 2,112.56 & 2,085.18 & 2,262.94 & 2,205.61 \\
Verifiable & 2,153.54 & 2,240.62 & 2,253.42 & 2,244.24 \\
Human-Verified & 1,922.49 & 1,986.74 & 1,976.66 & 1,945.26 \\
\midrule
\textbf{Average} & \textbf{2,123.00} & \textbf{2,133.68} & \textbf{2,270.22} & \textbf{2,193.38} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Average token usage per claim for full-context verification across benchmarks.}
\label{tab:fullcontext_tokens}
\begin{tabular}{lc}
\toprule
\textbf{Benchmark} & \textbf{Tokens per Claim} \\
\midrule
Golden Supported & 21,648.85 \\
Author--Reviewer & 21,130.27 \\
Paper + O4-mini & 21,130.27 \\
Agreement & 22,323.60 \\
Verifiable & 21,333.30 \\
Human-Verified & 18,912.43 \\
\midrule
\textbf{Average} & \textbf{21,079.79} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Token efficiency comparison: RAG-based vs. full-context verification. Reduction factor shows how many times fewer tokens RAG uses compared to full-context.}
\label{tab:comparison}
\begin{tabular}{lccc}
\toprule
\textbf{Benchmark} & \textbf{Full-Context} & \textbf{RAG (Avg)} & \textbf{Reduction Factor} \\
\midrule
Golden Supported & 21,648.85 & 2,285.96 & 9.47$\times$ \\
Author--Reviewer & 21,130.27 & 2,223.57 & 9.50$\times$ \\
Paper + O4-mini & 21,130.27 & 2,223.57 & 9.50$\times$ \\
Agreement & 22,323.60 & 2,166.57 & 10.30$\times$ \\
Verifiable & 21,333.30 & 2,222.96 & 9.60$\times$ \\
Human-Verified & 18,912.43 & 1,957.79 & 9.66$\times$ \\
\midrule
\textbf{Overall Average} & \textbf{21,079.79} & \textbf{2,180.07} & \textbf{9.67$\times$} \\
\bottomrule
\end{tabular}
\end{table}
